Linear spectro-polarimetry: a new diagnostic tool for the classification and characterisation of asteroids

We explore the use of spectro-polarimetry as a remote sensing tool for asteroids in addition to traditional reflectance measurements. In particular we are interested in possible relationships between the wavelength-dependent variation of linear polarization and the properties of the surfaces, including albedo and composition. We have obtained optical spectro-polarimetric measurements of a dozen asteroids of different albedo and taxonomic classes and of two small regions at the limb of the Moon. We found that objects with marginally different relative reflectance spectra (in the optical) may have totally different polarization spectra. This suggests that spectro-polarimetry may be used to refine the classification of asteroids. We also found that in some cases the Umov law may be violated, that is, in contrast to what is expected from basic physical considerations, the fraction of linear polarization and the reflectance may be positively correlated. In agreement with a few previous studies based on multi-colour broadband polarimetry, we found that the variation of linear polarization with wavelength and with phase-angle is correlated with the albedo and taxonomic class of the objects. Finally, we have serendipitously discovered that spinel-rich asteroid (599) Luisa, located very close to the Watsonia family, is a member of the rare class of Barbarian asteroids. We suggest that future modelling attempts of the surface structure of asteroids should be aimed at explaining both reflectance and polarization spectra.

==> Tab_BB.tex <==
\caption{\label{Tab_BB}
Values of the broadband linear polarization inferred from polarized spectra. Error
bars due to photon-noise are very small and not significant. Accuracy is determined
by residual instrumental polarization, which we estimate $\le 0.1$\,\%. Note that 
these values refer to the Bessel broadband filter used in FORS1.
}
\begin{small}
\begin{center}% 1234567
\begin{tabular}{llcrrrr}
\hline\hline
% 1234567
  &&&&&&\\
\multicolumn{1}{c}{Object}       &
\multicolumn{2}{c}{Class}        &
\multicolumn{1}{c}{$\alpha$}     &
\multicolumn{1}{c}{$ B $}    &
\multicolumn{1}{c}{$ V $}    &
\multicolumn{1}{c}{$ R $}    &
\multicolumn{1}{c}{$ I $}   \\
\multicolumn{1}{c}{}       &
\multicolumn{1}{c}{}       &
\multicolumn{1}{c}{}        &
\multicolumn{1}{c}{$(\%)$}    &
\multicolumn{1}{c}{$(\%)$}    &
\multicolumn{1}{c}{$(\%)$}    &
\multicolumn{1}{c}{$(\%)$}   \\
\hline
  &&&&&&&\\
%           & type   & alpha     &    B  &   V   &   R   &   I   \\
  (1) Ceres   & G & C  &$22.4\degr$&$     $&$ 1.17$&$ 1.21$&$ 1.25$\\ [2mm]
  (2) Pallas  & B & B  &$27.5\degr$&$ 2.21$&$ 2.25$&$ 2.29$&$ 2.33$\\ 
              &   &    &$22.9\degr$&$     $&$ 0.99$&$ 1.00$&$ 1.03$\\ [2mm]
  (7) Iris    & S & S  &$26.9\degr$&$     $&$ 0.58$&$ 0.52$&$ 0.48$\\
              &   &    &$27.5\degr$&$     $&$ 0.68$&$ 0.62$&$ 0.56$\\
              &   &    &$28.2\degr$&$ 0.89$&$ 0.75$&$ 0.68$&$ 0.64$\\ [2mm]
  (8) Flora   & S & S  &$28.4\degr$&$     $&$ 0.78$&$ 0.68$&$ 0.60$\\ [2mm]
 (21) Lutetia & M & Xc &$14.6\degr$&$-1.16$&$-1.19$&$-1.23$&$-1.23$\\ [2mm]
 (24) Themis  & C & B  &$14.0\degr$&$-1.26$&$-1.23$&$-1.18$&$-1.12$\\ [2mm]
 (44) Nysa    & E & Xc &$ 9.1\degr$&$     $&$-0.27$&$-0.30$&$-0.32$\\ [2mm]
              &   &    &$14.2\degr$&$     $&$     $&$     $&$     $\\ [2mm]
 (51) Nemausa &Cu & Ch &$15.7\degr$&$-1.18$&$-1.11$&$-1.10$&$-1.06$\\ [2mm]
(208) Lacrimosa&S & Sk &$13.7\degr$&$-0.46$&$-0.46$&$-0.47$&$-0.50$\\ [2mm]
(236) Honoria & S & L  &$ 7.1\degr$&$-0.91$&$-1.00$&$-1.08$&$-1.17$\\ [2mm]
(433) Eros    & S & S  &$42.0\degr$&$ 2.54$&$ 1.99$&$ 1.87$&$ 1.86$\\
(599) Luisa   & S & K  &$26.9\degr$&$-0.43$&$-0.39$&$-0.30$&$-0.16$\\ [2mm]
% (4) Vesta   &   & V  &$25.3\degr$&$ 0.31$&$ 0.26$&$ 0.22$&$ 0.24$\\ [2mm]
\hline
\end{tabular}
\end{center}
\end{small}

